Stochastic Model-Based Methods for Minimizing Paraconvex Functions

This paper studies stochastic algorithms for minimizing paraconvex functions, a function class that generalizes weakly convex functions and includes, for instance, H\"older smooth functions and compositions of convex functions with H\"older smooth maps. We first establish the convergence of the stochastic subgradient method and the stochastic proximal subgradient method for unconstrained and composite paraconvex optimization, respectively. The analysis is then extended to a broad family of algorithms that access the objective through stochastic models satisfying certain approximation-quality and continuity assumptions. The main principle that underlies the convergence analysis is that the algorithms under consideration can be interpreted as perturbed descent methods on the generalized Moreau envelope of the original paraconvex problem.

==> macros.tex <==
% argmin, argmax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

% esssup
\DeclareMathOperator*{\esssup}{ess\,sup}

% expectation of distance
\newcommand{\meandist}[3][]{\mathbb{E}_{#1}\left[\left\lVert#2 - #3\right\rVert^2\right]}

% E
\newcommand{\E}[2][]{\mathbb{E}_{#1}\!\left[#2\right]}
\newcommand{\EE}[0]{\mathbb{E}}

% norms
% Absolute value
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}

% norms
\newcommand{\norm}[2][]{\left\lVert #2 \right\rVert^{#1}}

% Total-variation norm
\newcommand{\normtv}[1]{\left\lVert #1 \right\rVert_{\mathrm{TV}}}

% Gradient estimator
\newcommand{\gradestimfull}[2][]{g_{#1} \left( x_{#2}; \boldsymbol{\xi}^{#1}_{#2}, K^{#1}_{#2} \right)}
\newcommand{\gradestim}[2][]{g_{#1} \left( x_{#2} \right) }
\newcommand{\meangradestim}[1]{ \bar{g} \left( x_{#1} \right) }

% Min & max
\newcommand{\mmin}[2][]{\underset{#1}{\min} \left\{ #2 \right\}}
\newcommand{\mmax}[2][]{\underset{#1}{\max} \left\{ #2 \right\}}
\newcommand{\margmin}[2][]{\underset{#1}{\argmin} \left\{ #2 \right\}}
\newcommand{\margmax}[2][]{\underset{#1}{\argmax} \left\{ #2 \right\}}

% Problem & algo class
\newcommand{\problemclass}[0]{\mathcal{F}}
\newcommand{\algoclassfull}[0]{\mathcal{A} \left( C^0_{\infty}, \left( C_{\infty}^m, \tau_m, V_m, V_{m, \pi}, B_m \right)_{m\in[M]} \right) }
\newcommand{\algoclass}[0]{\mathcal{A}_{\text{async}}}
\newcommand{\algoclasssync}[0]{\mathcal{A}_{\text{sync}}}

% Prox operator
\newcommand{\prox}[2][]{\operatorname{prox}_{#1} \left( #2 \right)}
\newcommand{\proj}[2][]{\operatorname{proj}_{#1} \left( #2 \right)}
\newcommand{\brho}[0]{\bar{\rho}}
\newcommand{\trho}[0]{\tilde{\rho}}

% Domain & epigraph
\newcommand{\dom}[1]{\text{dom}~ #1}
\newcommand{\epi}[1]{\text{epi}~ #1}

% Sets & Parentheses
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\pa}[1]{\left( #1 \right)}
\newcommand{\inn}[1]{\langle #1 \rangle}

% Number sets
\newcommand{\extr}[0]{\mathbb{R} \cup \{ +\infty \}} % extend real line
\newcommand{\rd}[1]{\mathbb{R}^{#1}} % R^d
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\N}[0]{\mathbb{N}}

% Distance to set
\newcommand{\dist}[2][]{\text{dist} \left( #1; #2 \right)}

% Balls
\newcommand{\unitball}[0]{\mathbf{B}}
\newcommand{\ball}[2][]{\mathbf{B} \left(#1, #2\right)}

% Generalized Moreau envelope and generalized proximal maping
\newcommand{\moreau}[1]{M^{p, r}_F \left( #1 \right)}
\newcommand{\gprox}[1]{P^{p, r}_F \left( #1 \right)}

\NewDocumentCommand{\moreaup}{O{r} O{F} m}{M^{#1}_{#2} \left( #3 \right)}
\NewDocumentCommand{\gproxp}{O{r} O{F} m}{P^{#1}_{#2} \left( #3 \right)}

\newcommand{\model}[2][]{f_{#1}(#2, \xi_t)}

% 

% Sample complexities
\newcommand{\sasmlmc}[0]{\mathcal{S}_{\text{Async MLMC}}}
\newcommand{\sasmini}[0]{\mathcal{S}_{\text{Async Mini}}}
\newcommand{\ssmlmc}[0]{\mathcal{S}_{\text{Sync MLMC}}}
\newcommand{\ssmini}[0]{\mathcal{S}_{\text{Sync Mini}}}
\newcommand{\rmlmcmini}[0]{\mathcal{R}^{\text{Async MLMC}}_{\text{Sync Mini}}}
\newcommand{\rmlmcmlmc}[0]{\mathcal{R}^{\text{Async MLMC}}_{\text{Sync MLMC}}}
\newcommand{\rminimini}[0]{\mathcal{R}^{\text{Async Mini}}_{\text{Sync Mini}}}
\newcommand{\rminimlmc}[0]{\mathcal{R}^{\text{Async Mini}}_{\text{Sync MLMC}}}

% C infinity
\newcommand{\cmax}[0]{C_{\infty}^{\max}}
\newcommand{\cinf}[0]{C_{\infty}}
\newcommand{\czero}[0]{C_{\infty}^0}


==> preamble.tex <==
% jota_shared.tex
% Shared preamble for the JOTA (svjour3) version.
% \input{jota_shared} right after \documentclass[...]{svjour3}.

% svjour3 raises "Extra \else" if microtype is loaded late
\RequirePackage{microtype}

% Flush-right end-of-proof box; JOTA requires \qed at the end of proofs
\smartqed

% Mathematics (svjour3 loads none of these)
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathtools} % for \coloneqq
\DeclareMathOperator{\diag}{diag}

% Figures & friends
\usepackage{graphicx}
\graphicspath{figures/}
\usepackage{epstopdf}
\usepackage{float}
\usepackage{xcolor}
\usepackage{subcaption}

% Algorithms: svjour3 has no algorithm float, siamart provided one
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{xparse}
\usepackage{etoolbox}

% Tables
\usepackage{booktabs}

% Theorem-like environments.
% With the class options envcountsame + envcountsect, svjour3 already defines
% theorem, lemma, proposition, corollary, definition, example, remark, proof,
% all on the theorem counter and numbered by section (Theorem 3.1, Lemma 3.2, ...).
% Only the environments siamart did not have are added here.
\makeatletter
\let\claim\relax
\let\endclaim\relax
\makeatother
\spnewtheorem{claim}[theorem]{Claim}{\bfseries}{\itshape}
\spnewtheorem{assumption}[theorem]{Assumption}{\itshape}{\rmfamily}
\spnewtheorem{hypothesis}[theorem]{Hypothesis}{\itshape}{\rmfamily}
\spnewtheorem{fact}[theorem]{Fact}{\itshape}{\rmfamily}

% Cross-referencing
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% All svjour3 environments step the shared counter "theorem", so cleveref would
% print "Theorem" for every label. Alias the counter inside each environment.
\newcommand{\jotacrefenv}[3]{%
  \crefname{#1}{#2}{#3}\Crefname{#1}{#2}{#3}%
  \AtBeginEnvironment{#1}{\crefalias{theorem}{#1}}}
\jotacrefenv{lemma}{Lemma}{Lemmas}
\jotacrefenv{proposition}{Proposition}{Propositions}
\jotacrefenv{corollary}{Corollary}{Corollaries}
\jotacrefenv{definition}{Definition}{Definitions}
\jotacrefenv{example}{Example}{Examples}
\jotacrefenv{remark}{Remark}{Remarks}
\jotacrefenv{claim}{Claim}{Claims}
\jotacrefenv{assumption}{Assumption}{Assumptions}
\jotacrefenv{hypothesis}{Hypothesis}{Hypotheses}
\jotacrefenv{fact}{Fact}{Facts}

% JOTA cites equations by number in parentheses only: (1), not Eq. (1)
\crefformat{equation}{#2(#1)#3}
\Crefformat{equation}{#2(#1)#3}
\crefrangeformat{equation}{#3(#1)#4--#5(#2)#6}
\Crefrangeformat{equation}{#3(#1)#4--#5(#2)#6}
\crefmultiformat{equation}{#2(#1)#3}{ and~#2(#1)#3}{, #2(#1)#3}{, and~#2(#1)#3}
\Crefmultiformat{equation}{#2(#1)#3}{ and~#2(#1)#3}{, #2(#1)#3}{, and~#2(#1)#3}

\Crefname{ALC@unique}{Line}{Lines}

% Optional: append \qed to every proof automatically (siamart behaviour).
% JOTA prefers closing text such as "The proof is complete." before the box,
% so either enable this or add \qed by hand.
% \AtEndEnvironment{proof}{\qed}

\input{macros}

% Front matter (svjour3 stores these; \maketitle prints them)
% \journalname{Journal of Optimization Theory and Applications}
% \journalname{}

\title{Stochastic Model-Based Methods for Minimizing Paraconvex Functions}
\titlerunning{Stochastic Model-Based Methods for Minimizing Paraconvex Functions}
\dedication{Dedicated to Professor Simeon Reich on the occasion of his 80th birthday}


\author{Tan Khiem Huynh \and Van Ngai Huynh}
\authorrunning{T.~K. Huynh, V.~N. Huynh}

\institute{Tan Khiem Huynh \at
  Inria, INSA Lyon \\ 
  6 Avenue des Arts, 69621 Villeurbanne, France \\
  \email{tan-khiem.huynh@inria.fr}
  \and
  Van Ngai Huynh \at
  Department of Mathematics and Statistics, University of Quy Nhon \\ 
  170 An Duong Vuong, Quy Nhon, Viet Nam \\
  \email{vanngaihuynh@gmail.com}}

\date{Received: date / Accepted: date}
